Real-Time Navigation for Bipedal Robots in Dynamic Environments

The popularity of mobile robots has been steadily growing, with these robots being increasingly utilized to execute tasks previously completed by human workers. For bipedal robots to see this same success, robust autonomous navigation systems need to be developed that can execute in real-time and respond to dynamic environments. These systems can be divided into three stages: perception, planning, and control. A holistic navigation framework for bipedal robots must successfully integrate all three components of the autonomous navigation problem to enable robust real-world navigation. In this paper, we present a real-time navigation framework for bipedal robots in dynamic environments. The proposed system addresses all components of the navigation problem: We introduce a depth-based perception system for obstacle detection, mapping, and localization. A two-stage planner is developed to generate collision-free trajectories robust to unknown and dynamic environments. And execute trajectories on the Digit bipedal robot's walking gait controller. The navigation framework is validated through a series of simulation and hardware experiments that contain unknown environments and dynamic obstacles.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

The popularity of mobile robots has been increasing, with more mobile robots taking over tasks previously completed by human workers. Bipedal robots have been a popular field of research, due to the large range of tasks they can be utilized in. The general humanoid shape of bipedal robots allows them to be better integrated into a society designed for humans. However, for bipedal robots to be fully integrated into society, robust autonomous navigation systems need to be designed. These autonomous navigation systems for bipedal robots are generally divided into three stages: perception, planning, and control. 

Perception is used for the collection and extraction of useful information from the environment. Gathering information about the local environment, obstacles, and any objects of interest. Additionally, tracking the position of the robot during navigation through localization. Planning utilizes the extracted information for decision making within the environment to achieve high level goals. Control then executes sequences of joint positions and actuator commands to successfully execute the given plan. 

It is only with the combination of perception, planning, and control into a single navigation framework in which bipedal robots can truly integrate into human society. 
In this paper we seek to implement a holistic bipedal robot navigation framework to enable exploration of unknown, dynamic environments. The three components of autonomous navigation – perception, planning, and control – are combined into a single navigation system. The perception system must be capable of extracting obstacle and environment structure information. This environment information must then used to generate maps of the local and global environment to be used for planning. A planning framework must generate global paths and local trajectories that are robust to discovered environment regions and dynamic obstacles. Furthermore, these trajectories must respect the kinematic and dynamic constraints of the robot to ensure safe and feasible navigation. Finally, these trajectories must be executed with a low-level controller that maintains safe and stable walking gaits. The combination of these capabilities will enable the safe navigation of bipedal robots in complex environments.



The rest of this paper is organized as follows. Sec. III introduces the navigation framework architecture, explaining the perception, mapping, localization, planning, and controller utilized. In Sec. IV, the simulation and hardware experiments are introduced and their results discussed. Finally, Sec. V concludes the navigation framework introduced, summarizes the experiments conducted, and limitations and future work are discussed. 

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}


...


The rest of this paper is organized as follows. Sec. III introduces the navigation framework architecture, explaining the perception, mapping, localization, planning, and controller utilized. In Sec. IV, the simulation and hardware experiments are introduced and their results discussed. Finally, Sec. V concludes the navigation framework introduced, summarizes the experiments conducted, and limitations and future work are discussed. 

==> sections/system_architecture.tex <==
\section{Navigation Framework Architecture}
\label{sec:architecture}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/system_overview.png}
    \caption{The proposed navigation framework. An architecture built on Move Base Flex \cite{8593829}, detections are made using RGB-D modules and a LiDAR sensor. The detections are used for obstacle segmentation by Random Sample Consensus \cite{Fischler_Bolles_1981}. The detected obstacles are used to generate global and local maps. LiDAR detections are used in LiDAR Odometry and Mapping \cite{Zhang-2017-110808} to localize the robot with respect to the global map. A goal position in the global environment is given to the robot. A D* Lite global planner \cite{d*lite} uses the global costmap to generate an optimal, collision-free path, which is used by the Timed-Elastic-Band local planner \cite{ROSMANN2017142} to generate local obstacle-avoiding trajectories. These trajectories are executed through velocity commands sent to Digit's walking gait controller.}
    \label{fig:system_architecture_overview}
\end{figure*}

\subsection{Perception}
The perception component of this framework relies on the sensor suite provided in the Digit bipedal robot. Digit is equipped with three depth modules (Intel RealSense D430), one RGB-Depth module (Intel RealSense D435), one color camera (The Imaging Source DFM 27UP), and one LiDAR sensor (Velodyne LiDAR Puck VLP-16). This navigation framework utilizes two of the depth modules and the LiDAR sensor. The two depth modules are placed at the pelvis, with one facing forwards at a downward angle and one facing rearwards at a downward angle. The LiDAR sensor is placed on top of Digit’s torso. The three sensors each provide a 3D point cloud which is streamed over a TCP/IP connection at an average rate of 14 Hz.

\subsection{Point Cloud Pre-processing}
The two depth modules obtain point clouds from directly in front and behind Digit. These point clouds are used to capture information about obstacles in the local environment. However, before extracting obstacle information, the raw point clouds from the depth modules must be pre-processed. 
Each depth module provides a very dense point cloud, causing later operations of obstacle segmentation, mapping, and localization to be computationally costly when using the raw point clouds. Both forward and rearward depth modules have a reliable detection range of 2.0-3.0 m, with detection accuracy dropping significantly past 3.0 m.

First, the point clouds from the depth modules are down sampled using a Voxel Grid filter as implemented in \cite{5980567}. A leaf size of 0.02 m per voxel dimension was chosen which adequately retains obstacle information while resulting in an average point cloud size reduction of 91.07\%. Additionally, to prevent inaccurate detection due to measurement distance, the point cloud is filtered to retain only points within 2.9 meters of each depth module. Furthermore, reflections can cause outlier points to be detected underground and outside of the range of the sensor. These points are filtered using a pass-through filter to remove NaN values and points with a height value below a specified threshold.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/obstacle_segmentation_digit.png}
    \caption{Results from point cloud pre-processing and obstacle segmentation. a) Shows the original point cloud, b) shows the filtered cloud, and c) shows the filtered point cloud with segmented obstacles in red.}
    \label{fig:obstacle_segmentation_digit}
\end{figure}

\subsection{Obstacle Segmentation}
After filtering the point cloud from both depth modules, the resulting clouds are fused into a combined point cloud. The Random Sample Consensus (RANSAC) method proposed in \cite{Fischler_Bolles_1981} is used to segment obstacles from the fused depth module point cloud. For a given point cloud, $P$, RANSAC randomly samples 3 points to solve a unique plane model,
\begin{equation}
    ax + by + cz + d = 0,
\end{equation}
where \({a,b,c,d}\in\mathbb{R}\) are the fitted coefficients, and $(x,y,z)\in\mathbb{R}^3$ represents the Cartesian coordinate of a point.
Then, the absolute distance, \(D_i\), of each point \(i\) in the cloud is calculated for the fitted model.
\begin{equation}
    D_i=\left|\frac{a x_i+b y_i+c z_i+d}{\sqrt{a^2+b^2+c^2}}\right|, \text { for } i \in\{1,2, . ., n\}
\end{equation}
where $n$, is the total number of points in the point cloud $P$.
Next, points within a given threshold distance, \(D_{threshold}\), to the plane model are labeled as inliers of the model, denoted \(P_I\),
\begin{equation}
    P_I=\left\{p_i \in P \mid D_i<D_{\text {threshold}}\right\}
\end{equation}
This process is repeated iteratively for a specified number of iterations, \(N\), determined statistically as: 
\begin{equation}
    N=round(\frac{\log{(1-\alpha)}}{\log{(1-(1-\epsilon)^3)}})
\end{equation}
where $\alpha$ is the desired minimum probability of finding at least one good plane from $P$, usually within \([0.90-0.99]\), and \(\epsilon=(1-u)\) where $u$ is the probability that any selected point is an inlier.
The resulting plane model is selected as the one which generates the largest number of inliers with the smallest standard deviation of distances.

Using the resulting plane model from RANSAC, outlier points of the plane model are segmented from the original point cloud and stored into an obstacle point cloud. The remaining points from the original point cloud are then considered the free space ground point cloud. The resulting obstacle and ground point clouds are then used for obstacle mapping. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/digit_map.png}
    \caption{Mapping results from the same environment as shown in \ref{fig:obstacle_segmentation_digit}. a) Shows the global map, capturing the entire environment, b) shows the local map which only captures local obstacles, and c) shows the overlaid global and local maps.}
    \label{fig:digit_mapping_example}
\end{figure}

\subsection{Mapping}
Two layered 2D costmaps presented in \cite{6942636} are used to store real-time information about the surrounding obstacles and environment. 
\subsubsection{Global Map}
As the robot navigates through the environment, long term mapping of environment obstructions and general environment structure is required. The purpose of the global map is not to track local, dynamic obstacles but rather capture and store macro-scale information of the environment. Compared to the local map, the global map is intended to map entire environments. To enable this, the global map uses a lower resolution of 0.1 m and only updates at a rate of 2 Hz. The global map is solely populated by detections from the LiDAR sensor. Cells in the global map have two possible states:
\paragraph{Occupied}
Any 3D point detections from the perception sensors are projected onto the 2D plane of the global map. Any cells that contain projected points are considered to be occupied by obstacles. All occupied cells are considered untraversable.
\paragraph{Free}
Any cell that is not occupied is considered free and traversable for the robot. Unexplored regions of the environment are by default considered to be free.
The global planner is deployed in the global map, while the local planner operates entirely in the local map.
\subsubsection{Local Map}
The local trajectory planner does not require the entirety of the environment information stored in the global map. Instead, the local map is designed to capture a small region of the environment local to the robot. In this framework, the local map is a 4 m x 4 m region with the origin at the robot's center of mass. The local map is not intended to store explored environment information, rather to capture local dynamic obstacles and facilitate real-time obstacle avoidance. To enable this the local map uses a higher resolution of 0.05 m and updates at a rate of 10 Hz. The local map is populated using detection from both the pre-processed obstacle point cloud and the LiDAR sensor. Similar to the global map, the local map cells can be in one of three possible states: Occupied, Free, and, Inflated. Occupied and Free cell states are identical to that of the global map.
\setcounter{paragraph}{2}
\paragraph{Inflated}
Cells within a certain distance of obstacles are inflated with non-zero cell costs. These non-zero costs are used to penalize trajectory planning through regions close to obstacles while not completely prohibiting trajectories from entering these regions.

\subsection{Localization}
LiDAR Odometry and Mapping (LOAM), a method introduced by J. Zhang and S. Singh in \cite{Zhang-2017-110808}, is used to estimate the odometry of the robot. LOAM introduces a two-part approach to simultaneous localization and mapping. The problem is divided into two separate simultaneously executed algorithms: one algorithm performs odometry estimation operations while the other performs mapping operations. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/LOAM_overview.png}
    \caption{Overview of the LiDAR Odometry and Mapping (LOAM) system as shown in \cite{Zhang-2017-110808}.}
    \label{fig:loam_overview}
\end{figure}
The LiDAR odometry algorithm runs at 10 Hz in which the correspondence of extracted features from consecutive LiDAR sensor sweeps are used to estimate the motion of the sensor. First, edge and planar features are extracted from the point cloud by assigning each point in the cloud a smoothness value, $c_i$:
\begin{equation}
    c_i=\frac{1}{|\mathcal{S}| \cdot\left\|\boldsymbol{X}_{(k, i)}^L\right\|} \cdot \sum_{j \in \mathcal{S}, j \neq i}\left(\boldsymbol{X}_{(k, i)}^L-\boldsymbol{X}_{(k, j)}^L\right),
\end{equation}
where \(\boldsymbol{X}_{(k, i)}^L\) and \(\boldsymbol{X}_{(k, j)}^L\) are the points $i$ and $j$ in the LiDAR coordinate system, $L$, received during the sensor sweep $k$, and \(\mathcal{S}\) is the set of consecutive points in a scan.
The points with the highest smoothness values are classified as edge points, and points with the lowest values are classified as planar points. To ensure an even distribution of features, a maximum of 2 edge points and 4 planar points are extracted from each of 4 identical subregions. 

At the end of each sweep, the accumulated point cloud, \(\mathcal{P}_k\), during the sweep is projected to time stamp \(t_{k+1}\) to generate point cloud, \(\overline{\mathcal{P}}_k\). The projected point cloud is used together with the point cloud accumulated during the next sweep \(\mathcal{P}_{k+1}\). Features are extracted from \(\mathcal{P}_{k+1}\) using the previously described method. Edge lines are found as the correspondence of points in the set of projected edge points, $\tilde{\mathcal{E}}_{k+1}$, and planar patches are found as the correspondence of points in the set of projected planar points, $\tilde{\mathcal{H}}_{k+1}$, between the projected cloud \(\overline{\mathcal{P}}_k\) and consecutive point cloud \(\mathcal{P}_{k+1}\). 

With correspondences found for the feature points, the distances between feature points and their correspondence can be found. For a point \(i\in\tilde{\mathcal{E}}_{k+1}\) who has a correspondence edge line $(j, l)$ with \(j, l \in \overline{\mathcal{P}}_k\), the point to line distance is:
\begin{equation}
    d_{\mathcal{E}}=\frac{\left|\left(\tilde{\boldsymbol{X}}_{(k+1, i)}^L-\overline{\boldsymbol{X}}_{(k, j)}^L\right) \times\left(\tilde{\boldsymbol{X}}_{(k+1, i)}^L-\overline{\boldsymbol{X}}_{(k, l)}^L\right)\right|}{\left|\overline{\boldsymbol{X}}_{(k, j)}^L-\overline{\boldsymbol{X}}_{(k, l)}^L\right|},
\end{equation}
and for a point \(i\in\tilde{\mathcal{H}}_{k+1}\) who has a correspondence planar patch $(j, l, m)$ with \(j, l, m \in \overline{\mathcal{P}}_k\), the point to patch distance is:
\begin{equation}
    d_{\mathcal{H}}=\frac{\left|\begin{array}{c}
\left(\tilde{\boldsymbol{X}}_{(k+1, i)}^L-\overline{\boldsymbol{X}}_{(k, j)}^L\right) \\
\left(\left(\overline{\boldsymbol{X}}_{(k, j)}^L-\overline{\boldsymbol{X}}_{(k, l)}^L\right) \times\left(\overline{\boldsymbol{X}}_{(k, j)}^L-\overline{\boldsymbol{X}}_{(k, m)}^L\right)\right)
\end{array}\right|}{\left|\left(\overline{\boldsymbol{X}}_{(k, j)}^L-\overline{\boldsymbol{X}}_{(k, l)}^L\right) \times\left(\overline{\boldsymbol{X}}_{(k, j)}^L-\overline{\boldsymbol{X}}_{(k, m)}^L\right)\right|},
\end{equation}
where \(\tilde{\boldsymbol{X}}_{(k+1, i)}^L, \overline{\boldsymbol{X}}_{(k, j)}^L, \overline{\boldsymbol{X}}_{(k, l)}^L\) are the coordinates of points $i$, $j$, and $l$ in the LiDAR coordinate system, respectively.
Using the correspondences, geometric relationships can be formed between an edge point and its corresponding edge line and a planar point and its corresponding planar patch:
\begin{equation}
    f_{\mathcal{E}}\left(\boldsymbol{X}_{(k+1, i)}^L, \boldsymbol{T}_{k+1}^L\right)=d_{\mathcal{E}}, i \in \mathcal{E}_{k+1},
\end{equation}
\begin{equation}
    f_{\mathcal{H}}\left(\boldsymbol{X}_{(k+1, i)}^L, \boldsymbol{T}_{k+1}^L\right)=d_{\mathcal{H}}, i \in \mathcal{H}_{k+1},
\end{equation}
where \(\boldsymbol{T}_{k+1}^L\) is the LiDAR pose transform from \([t_{k+1}, t]\), and $\mathcal{E}_{k+1}$ and $\mathcal{H}_{k+1}$ are the sets of edge points and planar points from $\mathcal{P}_{k+1}$.
These relationships are stacked for each edge feature point and each planar feature point to obtain a nonlinear function,
\begin{equation}
    \boldsymbol{f}\left(\boldsymbol{T}_{k+1}^L\right)=\boldsymbol{d},
\end{equation}
where each row of $\boldsymbol{f}$ is a feature point and each row of $\boldsymbol{d}$ is the correspondance distance.
which is solved with the Levenberg-Marquardt method \cite{Hartley:2003:MVG:861369} to obtain the motion estimation of the LiDAR sensor, which can then be used to retrieve the motion estimation of the robot.

\subsection{Planning}
\subsubsection{D* Lite global planner}
While the robot explores unknown environments, a global planner is needed to generate collision-free paths through the global map to reach a goal position. As the robot discovers new environment information, the planner must be capable of quick replanning to account for map updates. Therefore, a D* Lite global planner as presented in \cite{d*lite} is used to generate high level paths. D* Lite is a fast-replanning method designed to solve goal-directed navigation problems in environments modelled as eight-connected graphs. This planning method can be directly applied to the layered 2D costmaps described in Sec. III.D and allows for efficient replanning as the robot explores undiscovered environments.

The D* Lite planner assigns each explored cell, \(s\) in the costmap two values:
an estimate of the goal distance, g(s),
\begin{equation}
    g(s)=h(s, s_{start})
\end{equation}
where \(h\) is the Euclidean distance from the start cell \(s_{start}\) to the current cell \(s\), and a one-step lookahead value based on the g-value, \(rhs(s)\),
\begin{equation}
    rhs(s)= \begin{cases}0 & \text { if } s=s_{s t a r t} \\ \min _{s^{\prime} \in \operatorname{Pred}(s)}\left(g\left(s^{\prime}\right)+c\left(s^{\prime}, s\right)\right) & \text { otherwise }\end{cases}
\end{equation}
where \(c(s', s)\) is the cost to traverse to a neighboring cell \(s'\) from the current cell \(s\).

To calculate the shortest path, the planner begins from the goal position and explores towards the start position. All neighbors of the current cell are added to a priority queue with a key value:
\begin{equation}
    k(s) = [k_1(s), k_2(s)],
\end{equation}
with
\begin{equation}
    k_1(s) = \min(g(s), rhs(s)) + h(s, s_{start}) + k_m,
\end{equation}
\begin{equation}
    k_1(s) = \min(g(s), rhs(s)).
\end{equation}
The priority queue is sorted by the following: a key \(k(s) \leq k'(s)\) iff \(k_1(s) < k'_1(s)\) or \(k_1(s) = k'_1(s)\) and \(k_2(s) < k'_2(s)\).
The planner always expands the low-valued cell in the priority queue. The successor cells, or neighbors, of this top-most cell have their \(g\) and \(rhs\) values updated and then are added to the priority queue. This process continues until the expanded cell is the start position or all possible cells have been expanded. 

The main planning algorithm initially calculates the shortest path as previously described based on the initial environment information. As the robot follows the generated path and new environment areas are explored and obstacles are detected, the costmap is updated to reflect the new detections and the global planner re-calculates the global path as previously described. If a path exists, D* Lite ensures that the shortest path can be followed by always moving from the current position cell \(s\), starting from the starting position \(s_{start}\), and traversing to the successor cell \(s’\) that minimizes \(c(s, s’) + g(s’)\).
The global planner returns a sequence of waypoint cells within the global costmap to follow and are updated at a rate of 5 Hz. 

\subsubsection{Timed-Elastic-Band local planner}
The purpose of the local planner is to generate a smooth, kinematically feasible trajectory that follows the global path generated by the D* Lite global planner. The Timed-Elastic-Band method introduced in \cite{ROSMANN2017142} originally implements a trajectory optimization method for differential drive and carlike robots. We adapted for use in bipedal robots by applying simplifying assumptions on the high-level kinematic constraints of the low-level controller to mimic those of a differential drive robot. The bipedal locomotion is modelled as a differential drive model to avoid several problems introduced from the unique ability for omnidirectional movement of bipedal robots. For example, lateral velocity in bipedal locomotion is difficult to control due to oscillating behaviors in the lateral direction. The Timed-Elastic-Band problem is defined as an open-loop optimization task to find the sequence of controls needed to move the robot from an initial pose \(\mathbf{s}_s\) to a goal pose \(\mathbf{s}_f\). This sequence of controls must execute in minimal time while maintaining the kinematic constraints of the robot and maintaining safe distances from obstacles.

Let \(\mathbf{s}_k =[x_k, y_k, \beta_k]^{\top}\) denote the robot pose at time \(k\). \(x_k\) and \(y_k\) denote the \(x\) and \(y\) position of the robot and \(\beta_k\) denotes the orientation of the robot. A trajectory is defined as a sequence of robot poses \(\mathcal{S} = \{\mathbf{s}_k | k = 1, 2, …, n\}\). The Timed-Elastic-Band planner then augments the trajectory with positive time intervals \(\Delta T_k, k = 1, 2, …, n\). The sequence of robot poses and time intervals are joined to form the parameter vector \(\mathbf b\):
\begin{equation}
    \mathbf{b}=\left[\mathbf{s}_1, \Delta T_1, \mathbf{s}_2, \Delta T_2, \mathbf{s}_3, \ldots, \Delta T_{n-1}, \mathbf{s}_n\right]^{\top}
\end{equation}
The optimization task is then defined as a nonlinear minimization task:
\begin{equation}\label{eq:loam_nonlinear_task}
    V^*(\mathbf{b})=\min_{\mathbf{b}}{\sum_{k=1}^{n-1} \Delta T_k^2}
\end{equation}
Which is subject to several constraints defined as equality and inequality constraints.

\paragraph{Non-holonomic constraint}
An equality constraint \(\mathbf{v}_k\) enforces the kinematic constraints of the robot. According to \cite{Rsmann2012TrajectoryMC} this non-holonomic constraint can be defined with a geometric interpretation to assume the robot can only execute smooth paths with consecutive poses \(\mathbf{s}_k\) and \(\mathbf{s}_{k+1}\) sharing a common arc of constant curvature. To enforce this constraint the angle \(\mathbf{\vartheta}_k\) between pose \(\mathbf{s}_k\) and direction \(\mathbf{d}_{k, k+1} = [x_{k+1}-x_k, y_{k+1}–y_k, 0]^{\top}\) has to be equal to the similar angle \(\vartheta_{k+1}\) at pose \(\mathbf{s}_{k+1}\),
\begin{equation}
    \vartheta_k = \vartheta_{k+1}
\end{equation}
\begin{equation}
    \begin{bmatrix}
        \cos (\beta_k) \\
        \sin (\beta_k) \\
        0
    \end{bmatrix} \times \mathbf{d}_{k, k+1} = \mathbf{d}_{k, k+1} \times \begin{bmatrix}
        \cos (\beta_{k+1}) \\
        \sin (\beta_{k+1}) \\
        0
    \end{bmatrix}
\end{equation}
and thus the resulting equality constraint applied to the optimization task in \eqref{eq:loam_nonlinear_task} is given by:
\begin{equation}
    \mathbf{h}_k(\mathbf{s}_{k+1}, \mathbf{s}_k) = \begin{pmatrix}
        \begin{bmatrix}
            \cos (\beta_k) \\
            \sin (\beta_k) \\
            0
        \end{bmatrix} + \begin{bmatrix}
            \cos (\beta_{k+1}) \\
            \sin (\beta_{k+1}) \\
            0
        \end{bmatrix}
    \end{pmatrix} \times \mathbf{d}_{k, k+1}. 
\end{equation}
\paragraph{Velocity and Acceleration constraints}
Additionally, limitations of the linear and angular velocities and accelerations are applied. First, the linear and angular velocities are approximated between two consecutive poses \(s_k\) and \(s_{k+1}\):
\begin{equation}
    v_k=\Delta T_k^{-1}\lVert [x_{k+1}-x_k, y_{k+1}-y_k]^{\top} \rVert\gamma(\mathbf{s}_k,\mathbf{s}_{k+1})
\end{equation}
\begin{equation}
    \omega_k=\Delta T_k^{-1}(\beta_{k+1}-\beta_k).
\end{equation}
Where \(\gamma(\mathbf{s}_k,\mathbf{s}_{k+1})\) is a sign extraction function which is approximated by a smooth sigmoidal approximation that maps to the interval \([-1, 1]\):
\begin{equation}
    \gamma(\mathbf{s}_k,\mathbf{s}_{k+1}) \approx \frac{\kappa \langle \mathbf{q}_k, \mathbf{d}_{k, k+1} \rangle}{1 + | \kappa \langle \mathbf{q}_k, \mathbf{d}_{k, k+1} \rangle |}
\end{equation}
Next, the linear and angular accelerations are approximated in a similar manner to the velocities between consecutive poses:
\begin{equation}
    a_k=\frac{2(v_{k+1}-v_k)}{\Delta T_k + \Delta T_{k+1}}
\end{equation}
\begin{equation}
    \dot{\omega}_k=\frac{2(\omega_{k+1}-\omega_k)}{\Delta T_k + \Delta T_{k+1}}
\end{equation}
Finally, the optimization task in \eqref{eq:loam_nonlinear_task} is constrained by the two inequalities:
\begin{equation}
    \mathbf{v}_k(\mathbf{s}_{k+1}, \mathbf{s}_{k}, \Delta T_k)=[v_{max}-|v_k|, \omega_{max}-|\omega_k|]^{\top}
\end{equation}
\begin{equation}
    \boldsymbol{\alpha}_k(\mathbf{s}_{k+2}, \mathbf{s}_{k+1}, \mathbf{s}_{k}, \Delta T_{k+1}, \Delta T_{k}))=[a_{max}-|a_k|, \dot\omega_{max}-|\dot\omega_k|]^{\top}
\end{equation}
As the velocity constraint and acceleration constraints respectively.

Furthermore, local planning must generate collision-free trajectories in obstacle-filled environments. The local planner considers obstacles, \(\mathcal{O}_l, l=1, 2, ..., R\), as simply-connected regions in the form of points, circles, polygons, and lines in \(\mathbb{R}^2\). To ensure a minimum separation \(\rho_{min}\) between pose \(\mathbf{s}_k\) and all obstacles, the inequality constraint applied to \eqref{eq:loam_nonlinear_task} is:
\begin{align}
    \begin{split}
        \mathbf{o}_k(\mathbf{s}_k)=[\rho(\mathbf{s}_k, \mathcal{O}_1), \rho(\mathbf{s}_k, \mathcal{O}_2), ..., \rho(\mathbf{s}_k, \mathcal{O}_R)]^{\top} \\
        - [\rho_{min}, \rho_{min}, ..., \rho_{min}]^{\top},
    \end{split}
\end{align}
where \(\rho\) is the minimal Euclidean distance between the obstacle and the robot pose. To simplify this calculation, the minimal distance is calculated from the obstacle to a circular safety region centered on the robot base frame with a radius of 0.25 m. 

The nonlinear task shown in \eqref{eq:loam_nonlinear_task} is computationally expensive to solve directly. Thus, the problem is transformed into an approximate nonlinear least-squares optimization problem that can be more efficiently solved. The constraints are applied to the approximated objective function as described in \cite{Nocedal_Wright}. The kinematic equality constraint is expressed as:
\begin{equation}
    \phi(\mathbf{h}_k, \sigma_h)=\sigma_h\lVert\mathbf{h}_k\rVert_2^{2},
\end{equation}
and the inequality constraints are approximated as:
\begin{equation}
    \chi(\mathbf{v}_k, \sigma_v)=\sigma_v\lVert\min\{\mathbf{0}, \mathbf{v}_k\}\rVert_2^{2},
\end{equation}
\begin{equation}
    \chi(\boldsymbol{\alpha}_k, \sigma_{\alpha})=\sigma_{\alpha}\lVert\min\{\mathbf{0}, \boldsymbol{\alpha}_k\}\rVert_2^{2},
\end{equation}
\begin{equation}
    \chi(\mathbf{o}_k, \sigma_o)=\sigma_o\lVert\min\{\mathbf{0}, \mathbf{o}_k\}\rVert_2^{2},
\end{equation}
where \(\sigma_i, i \in \{\mathbf{h}, \mathbf{v}, \boldsymbol{\alpha}, \mathbf{o}\}\) are scalar weights and the min operator is applied row-wise. 
The overall optimization problem is approximated with the objective function: 
\begin{equation}\label{eq:loam_kin_constraint_approx_1}
    \mathbf{b}^*=\argmin_{\mathcal{B}\backslash\{\mathbf{s}_1,\mathbf{s}_n\}} \tilde{V}(\mathbf{b})
\end{equation}
\begin{align}\label{eq:loam_kin_constraint_approx_2}
    \begin{split}
        \tilde{V}(\mathbf{b})=\sum_{k=1}^{n-1}[\Delta T_k^2 + \phi(\mathbf{h}_k, \sigma_h) + \chi(r_k, o_k) + ... \\ 
        + \chi(\mathbf{v}_k, \sigma_v) + \chi(\boldsymbol{\alpha}_k, \sigma_{\alpha}) + \chi(\mathbf{o}_k, \sigma_o)] + \chi(\boldsymbol{\alpha}_n, \sigma_{\alpha})
    \end{split}
\end{align}
This optimization problem is solved using a variant of the Levenberg–Marquardt algorithm implemented in the open-source graph optimization framework g2o \cite{Kmmerle2011G2oAG}.

As described in \cite{ROSMANN2017142} the Timed-Elastic-Band planner further improves the method by optimizing several of these trajectories from distinctive topologies in parallel to search for the global minimum of \eqref{eq:loam_nonlinear_task} resp. \eqref{eq:loam_kin_constraint_approx_1}.

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/turtlebot_static_5_7_tile_small.png}
    \caption{Experiment \ref{sssec:sim_exp_1}): The navigation framework executing on the Turtlebot3 differential drive robot. An initial goal is provided in a static environment. As unknown obstacles are discovered, re-planning occurs. Mid-way through execution, a new goal is provided and is reached.}
    \label{fig:sim_static_experiment_1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/turtlebot_dynamic_5_7_tile_small.png}
    \caption{Experiment \ref{sssec:sim_exp_2}): The navigation framework executing on the Turtlebot3 differential drive robot. An initial goal is provided in a dynamic environment. As the unknown dynamic obstacles is discovered, the robot stops, begins to reverse, and then plans around the obstacle. Once the dynamic obstacle has passed, the robot navigates to the goal.}
    \label{fig:sim_static_experiment_2}
\end{figure*}

\subsection{Controller}
The final output from the Timed-Elastic-Band planner is sequences of velocity commands to achieve the globally optimal trajectory \(\mathbf{b}^*\) from \eqref{eq:loam_kin_constraint_approx_1}. These velocity commands are sent to Digit’s default low-level controller provided by Agility Robotics.

